Complexity Results and Algorithms for Bipolar Argumentation

Bipolar Argumentation Frameworks (BAFs) admit several interpretations of the support relation and diverging definitions of semantics. Recently, several classes of BAFs have been captured as instances of bipolar Assumption-Based Argumentation, a class of Assumption-Based Argumentation (ABA). In this paper, we establish the complexity of bipolar ABA, and consequently of several classes of BAFs. In addition to the standard five complexity problems, we analyse the rarely-addressed extension enumeration problem too. We also advance backtracking-driven algorithms for enumerating extensions of bipolar ABA frameworks, and consequently of BAFs under several interpretations. We prove soundness and completeness of our algorithms, describe their implementation and provide a scalability evaluation. We thus contribute to the study of the as yet uninvestigated complexity problems of (variously interpreted) BAFs as well as of bipolar ABA, and provide the lacking implementations thereof.

==> figures/system.tex <==
\section{Implementation}
\label{sec:implementation}

We now discuss our implementation of the algorithms described in the previous section. Our tool aims to be more versatile than existing systems which almost exclusively focus on reasoning with AFs. In addition to directly enumerating extensions of bipolar ABA frameworks, our system is also capable of calculating extensions of AFs, BAFs and AFNs by utilising the existence of extension-preserving mappings from these formalisms into bipolar ABA.

We now describe the control flow of our system, as depicted graphically in figure \ref{fig:control-flow-diagram}.
\begin{enumerate}
    \item \textbf{Input argumentation framework.} The user inputs an argumentation framework to the system and specifies which semantics they would like the system to calculate extensions under. The argumentation framework can be an AF, BAF (necessary), BAF (deductive) or bipolar ABA framework.

\item \textbf{Parse argumentation framework.} The system parses the input and generates an internal representation of the input framework. 
\item \textbf{Perform standard mapping.} If the input framework is not a bipolar ABA framework, the system transforms it into a bipolar ABA framework using the mappings defined in \cite{Cyras:Schulz:Toni:2017}.
\item \textbf{Perform labelling algorithms.} The bipolar ABA framework is inputted to the labelling algorithms defined in section \ref{sec:algorithms}.
\item \textbf{Output Extensions.} Our system terminates after outputting the extensions calculated by the labelling algorithms. 

\end{enumerate} 
\begin{figure}[h]
\centering
  \includegraphics[width=0.75\linewidth]{figures/control-flow-diagram.pdf}
  \caption{Control flow diagram of our system.}
  \label{fig:control-flow-diagram}
\end{figure}

\subsubsection{Evaluation} \label{subsubsec:evaluation}
In order to test the scalability of our system, we generated 405 bipolar ABA frameworks of increasing size. To do this we adapted an existing benchmark generator from \cite{implementation-craven-argument-graphs}, originally used to create flat ABA frameworks, and adapted it to ensure that bipolar ABA frameworks are generated instead.
    
We input a tuple of parameters $(N_s, N_a, N_{rh}, N_{rph})$ to the generator in order to create our frameworks, the parameters are defined as follows.
\begin{enumerate}
    \item $N_s$ is the total number of sentences in the framework, i.e., $|\mathcal{L}|$.
    \item $N_ a$ is the number of assumptions, i.e., $|\mathcal{A}|$, given as a percentage of the number of sentences.
    \item $N_ {rh}$ is the number of distinct sentences to be used as rule heads, given as an integer.
    \item $N_ {rph}$ is the number of rules per distinct rule head, given as an interval [min, max], where min and max are integers.
\end{enumerate}

The specific parameters used to generate the frameworks were $(N_s , 37\%, N_s /2, [2, N_s /8]$) with the value of $N_s$ starting at 16, and increasing by 8 between subsequent frameworks. The largest frameworkx generated consisted of 3248 sentences, 1202 assumptions and 174,365 rules. 

We measured the elapsed time between inputting a framework to our system and our system outputting the extensions of that framework, under the admissible, preferred and set stable semantics, for all generated frameworks. The results are summarised in figure \ref{fig:experiment}.

\begin{figure}[h]
  \includegraphics[width=\linewidth]{figures/experiments_results}
  \caption{Elapsed time of our algorithm for calculating extensions of bipolar ABA frameworks.}
  \label{fig:experiment}
\end{figure}
The results show that even for the largest frameworks considered, our algorithms calculate extensions in under 30 seconds. We do see the performance begin to deteriorate as the size of the frameworks increase. This is expected since the backtracking method we rely on operates in $\mathcal{O}(2^n)$ in the worst case. Overall, we believe these results demonstrate the feasibility of our algorithms as a means of generating extensions of large argumentation frameworks.
